Evaluating Instruction-Tuned Large Language Models on Code Comprehension and Generation

In this work, we evaluate 10 open-source instructed LLMs on four representative code comprehension and generation tasks. We have the following main findings. First, for the zero-shot setting, instructed LLMs are very competitive on code comprehension and generation tasks and sometimes even better than small SOTA models specifically fine-tuned on each downstream task. We also find that larger instructed LLMs are not always better on code-related tasks. Second, for the few-shot setting, we find that adding demonstration examples substantially helps instructed LLMs perform better on most code comprehension and generation tasks; however, the examples would sometimes induce unstable or even worse performance. Furthermore, we find widely-used BM25-based shot selection strategy significantly outperforms the basic random selection or fixed selection only on generation problems. Third, for the fine-tuning setting, we find that fine-tuning could further improve the model performance on downstream code comprehension and generation tasks compared to the zero-shot/one-shot performance. In addition, after being fine-tuned on the same downstream task dataset, instructed LLMs outperform both the small SOTA models and similar-scaled LLMs without instruction tuning. Based on our findings, we further present practical implications on model and usage recommendation, performance and cost trade-offs, and future direction.

==> sections/approach.tex <==


\section{Approach} \label{sec:Approach}






==> sections/rq3.tex <==
\subsection{\llm{} Instruction Following Capability (RQ3)}
In this experiment, we focus to evaluate the \llm{} instruction following capability in the zero-shot and one-shot.
Specifically, when feeding a prompt to the \llm{}, there is a possibility that it may produce unexpected behavior by not adhering to the instructions provided in the prompt when generating a response.
For tasks other than CS, we establish specific rules to determine whether the output of the \llm{} conforms to the given instructions. 
Here, we do not evaluate the \llm{}'s instructions following ability at the CS task.
This is because the task requires \llm{} to generate natural language, which can have various forms. 
We cannot determine whether the generated natural language text adheres to the instructions through rule-based judgments.
For the other three tasks, we use the following rules to determine whether the output of the \llm{} follows the instructions.

\textit{DD \& CD}: Determine whether the output of \llm{} is YES or NO. 
If so, the \llm{} follows the instruction for the current output; otherwise, it does not follow the confluent instruction.
Here we are insensitive to the case of YES and NO.

\textit{AG}: Determine whether the output of the \llm{} contains an assertion code written using the Junit API. 
If so, the \llm{} follows the instruction for the current output; otherwise, it does not follow the confluent instruction.
It is worth noting that we focus solely on whether the \llm{} generates a line of assertion code using Junit, rather than examining for syntax errors in it.

\paragraph{\textbf{Result Analysis}}
\input{tables/instructionFollowing}
Table~\ref{table:instructioncompare} shows the \llm{}s' instruction-following capability in both zero-shot and one-shot scenarios.
In the zero-shot scenario, \llm{}s without instruction tuning exhibit poor instruction compliance compared to those with instruction tuning. 
For instance, \codegen{}'s instruction compliance on DD tasks is only 0.4\%.
When considering understanding tasks (DD and CD), the \llama{}-based \llm{}s (\vicuna{}, \alpaca{}, \codealpaca{}) demonstrate superior abilities in instructions following  compared to other architecture-based models (e.g., \dolly{} based on Pythia-6.9B). 
Specifically, \vicuna{}, \alpaca{}, and \codealpaca{} achieve close to 100\% compliance, while \dolly{} scores around 60\%.
As the \llm{} parameters increases, \dolly{}'s instruction following also increases, but \vicuna{}'s instruction following decreases on DD and CD.
This is primarily due to \vicuna{}-13B's tendency to provide responses with sentences that are more consistent with natural language characteristics instead of simple ``YES'' or ``NO'' answers. 
For example, in CD task, the responses could be ``There is no direct relationship ...'' or ``There is a relationship ...''.

Upon comparing the instruction-following ability of \llm{}s between the zero-shot and one-shot scenarios, we observe that adding a demonstrative example to the prompt effectively enhances the \llm{}'s ability to follow instructions. 
This improvement is evident not only in \llm{}s that have undergone instruction tuning but also in \llm{}s without instruction tuning. 
For instance, in the DD task, \chatglm{} shows an 82.0\% improvement in the BO scenario over the ZO scenario, while \codegen{}'s instruction following ability in the BO scenario increased by 77.4\% compared to the ZO scenario. 
This indicates that incorporating a demonstrative example in the prompt can effectively standardize response patterns and thus enhance the \llm{}'s instruction following capability.


\finding{Incorporating a demonstration example into the prompt has proven to be highly effective in enhancing the \llm{}'s instruction-following ability.
Even for \llm{} that have not undergone instruction tuning, the addition of an example in the prompt allows them to generate responses in a more standardized format.}




==> sections/rq4.tex <==
\subsection{RQ3: Costs}







==> tables/INSTRUCT.tex <==
\begin{comment}
\begin{table}[htb]
% \vspace{-2mm}
	\centering
	\small
	\caption{Average Instruction Following Performance}\label{table:instructionCompar}
	
	\begin{adjustbox}{width=0.70\columnwidth}
	   	
	\begin{tabular}{c|c|c}
		\hline
        \textbf{\llm{}} & \textbf{Zero-shot (\%)}  &  \textbf{One-shot (\%)}  \\ \hline  
        {\vicuna{}} & 94.3 & 97.7 \\ 
        {\alpaca{}} & \textbf{98.9} & 97.8 \\
        {\dolly{}} & 46.7 & 94.7 \\
        {\stablelm{}} & 70.3 & 94.7 \\
        {\chatglm{}} & 49.1 & \textbf{98.4} \\ 
        {\codealpaca{}} & 67.9 & 87.3 \\
        {\codegen{}} & 0.1 & 93.0 \\ 
        
        \hline
	\end{tabular}
	\end{adjustbox}
 % \vspace{-5mm}
\end{table}
\end{comment}

==> tables/largeLLM.tex <==

   
% \begin{table}[htb]
%     \centering
%     \caption{Large \llm{} Size Performance on Multi-task}\label{table:largeModel}
%     \begin{adjustbox}{width=1.0 \columnwidth}
%     \begin{tabular}{c|c|c|c|c|c|c|c|c}
%         \hline
%         \multirow{2}{*}{\textbf{Task}} & \multicolumn{2}{c|}{\textbf{{\vicuna{}-13B} (\%)}}  &  \multicolumn{2}{c|}{\textbf{\dolly{}-v2-12B (\%)}} &  \multicolumn{2}{c|}{\textbf{\wizardcoder{}-15B (\%)}} &  \multicolumn{2}{c}{\textbf{Instruct-\codegen{}-16B (\%)}}  \\  \cline{2-9} 
%         ~ & ZO & BO & ZO & BO & ZO & BO & ZO & BO  \\ \hline
%         DD & 49.8 & 49.2 & 46.9 & 47.4 & 52.6 & 53.1 & 23.0 & 53.6   \\ \hline
%         CD & 14.1 & 6.5 & 23.7 & 18.0 & 23.8 & 0.7 & 20.0 & 20.7 \\ \hline
%         AG & 12.0 & 44.0 & 1.0 & 51.7 & 19.4 & 63.3 & 2.9 & 53.9 \\  \hline
%         CS & 3.0 & 3.9  & 1.5 & 2.6 & 4.9 & 12.8 & 1.7 & 3.9   \\  \hline
%     \end{tabular}
%     \end{adjustbox}
% \end{table}

\begin{comment}

\begin{table}[htb]
    \centering
    \caption{The Larger \llm{} Performance on Multi-task}\label{table:largeModel}
    \begin{adjustbox}{width=1.0 \columnwidth}
    \begin{tabular}{c|>
    {\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.5cm}}
        \hline
        \multirow{2}{*}{\textbf{Task}} & \multicolumn{2}{c|}{\textbf{{\vicuna{}-13B} (\%)}}  &  \multicolumn{2}{c|}{\textbf{\dolly{}-v2-12B (\%)}} &  \multicolumn{2}{c|}{\textbf{\wizardcoder{}-15B (\%)}} &  \multicolumn{2}{c}{\textbf{Instruct-\codegen{}-16B (\%)}}  \\  \cline{2-9}
        ~ & ZS & BO & ZS & BO & ZS & BO & ZS & BO  \\ \hline
        DD & 49.8 & 49.2 & 46.9 & 47.4 & 52.6 & 53.1 & 23.0 & 53.6   \\ \hline
        CD & 14.1 & 6.5 & 23.7 & 18.0 & 23.8 & 0.7 & 20.0 & 20.7 \\ \hline
        AG & 12.0 & 44.0 & 1.0 & 51.7 & 19.4 & 63.3 & 2.9 & 53.9 \\  \hline
        CS & 71.0 & 52.0  & 63.0 & 45.0 & 9.0 & 13.0 & 5.0 & 9.0   \\  \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

    
\end{comment}





